IMU-Aided Event-based Stereo Visual Odometry

Direct methods for event-based visual odometry solve the mapping and camera pose tracking sub-problems by establishing implicit data association in a way that the generative model of events is exploited. The main bottlenecks faced by state-of-the-art work in this field include the high computational complexity of mapping and the limited accuracy of tracking. In this paper, we improve our previous direct pipeline \textit{Event-based Stereo Visual Odometry} in terms of accuracy and efficiency. To speed up the mapping operation, we propose an efficient strategy of edge-pixel sampling according to the local dynamics of events. The mapping performance in terms of completeness and local smoothness is also improved by combining the temporal stereo results and the static stereo results. To circumvent the degeneracy issue of camera pose tracking in recovering the yaw component of general 6-DoF motion, we introduce as a prior the gyroscope measurements via pre-integration. Experiments on publicly available datasets justify our improvement. We release our pipeline as an open-source software for future research in this field.

==> floats/alg_example.tex <==
%% Algorithm
\setlength{\textfloatsep}{2pt}
\begin{algorithm}[t]
% \setlength{\textfloatsep}{1pt}
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{Feature correspondence set $\mathcal{F}$, threshold $\mu$}
\Output{Feature labeling $\mathcal{L}_\text{f}$, model instance $\mathcal{M}$} 
\text{Initialize} $\mathcal{L}_\text{f} = \varnothing$, $\mathcal{M} = \varnothing$, $\omega^{\star} = 0$, $\bar{I} = \vert \cS \vert + 2$\\
$\mathcal{G} \leftarrow \text{Neighbourhood graph } (\mathcal{F})$\\
\While(\Comment*[f]{\text{Prog-X Loop}~\cite{Barath2019iccv}}){$\bar{I} > \vert \cS \vert + 1$}
{
\For(\Comment*[f]{\text{GC-RANSAC Loop}~\cite{barath2018graph}}){$k = 1 \text{ to } K$}
{
$\mathcal{S}$ $\leftarrow$ $\text{Sampled by NAPSAC}$ \cite{torr2002napsac}\\
$\mathbf{m}_h \leftarrow \text{Linear model fitting } (\mathcal{S})$\\
$\omega \leftarrow \text{Compute support of } \mathbf{m}_h $ (Eq.~\ref{eq:qualifying function})\\
\While{$\omega > \omega^{\star}$}{
$\omega^{\star} \leftarrow \omega$, $\mathbf{m}_h^{\star} \leftarrow \mathbf{m}_h$, $\mathcal{I}^{\star} \leftarrow \mathcal{I}$\\
% $\omega^{\star} \leftarrow \omega$\\
% $\mathcal{G} \leftarrow \text{Neighbourhood graph } (\mathcal{F})$\\
$\mathcal{I} \leftarrow  \text{Graph-Cut } (\mathbf{m}_h, \mathcal{G})$\\
$\mathbf{m}_h \leftarrow \text{Nonlinear model fitting }(\mathcal{I}$)\\
$\omega \leftarrow \text{Compute support of } \mathbf{m}_h $ (Eq.~\ref{eq:qualifying function})\\
% \If{$\omega > \omega^{\star}$}{
% $\omega^{\star} \leftarrow \omega$, $\mathbf{m}_h^{\star} \leftarrow \mathbf{m}_h$, 
% $\mathcal{I}^{\star} \leftarrow \mathcal{I}$\\}
}
}
$\cM \leftarrow \cM \oplus \mathbf{m}_h^{\star}$\\
$\{\mathcal{L}_\text{f}, \mathcal{M}\} \leftarrow \text{PEARL} (\cM, \mathcal{F})$~\cite{isack2012energy}\\
$\bar{I} \leftarrow \text{Compute the upper limit of } \vert \mathcal{I}^{\star} \vert $ (Eq.~\ref{eq:prog-x termination criteria})
}
\caption{Algorithm Example}
\label{alg: event clustering with prog-x}
\vspace{-1.5em}
\end{algorithm}



==> floats/fig_imu_benefit.tex <==
\begin{figure}[ht]
\centering
\subfigure[part of city\_04\_a]{\includegraphics[width=0.23\textwidth]{img/IMU/a.png}}\hspace{0pt}
\subfigure[part of city\_04\_c]{\includegraphics[width=0.23\textwidth]{img/IMU/c.png}}
\caption{\textit{Comparison of w/o IMU and w/ IMU.} 2D trajectory estimates for the \textit {zurich\_city\_04} sequences from DSEC dataset.The ground truth trajectory is provided by LiDAR. Results of ground truth are depicted in black, w/o IMU in green, and w/ IMU in blue. The figures show trajectories with aligned.}
\label{fig:IMU benefit}
\vspace{-1.5em}
\end{figure}

==> floats/fig_mapping_flowchart.tex <==
\begin{figure}[ht]
    \centering
    % \hspace{5pt}\includegraphics[width=0.48\textwidth]{img/fusion.png}
    \caption{\textit{Mapping thread.}
    \textcolor{red}{To replace this figure.}}
    \label{fig:mapping module}
\vspace{-1.5em}
\end{figure}

==> floats/flowchart_example.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{img/RAL_Cascaded_flowchart.pdf}
   \captionof{figure}{Flowchart example.}
  \label{fig:flowchart}
\end{figure*}


==> floats/tab_dataset.tex <==
\begin{table}[t]
\vspace{-0em}
\begin{center}
\caption{Parameters of various stereo event-camera rigs used in the experiments.}
\vspace{0em}
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ccccc}
\hline
{Dataset} & {Cameras} & {Resolution(pix)} & {Baseline(cm)} & {FOV($^\circ$)}\\
\hline
{\cite{Zhou18eccv}} & {DAVIS240C} & {240 × 180} & {14.7} & {62.9}\\
{\cite{Gehrig21ral}} & {Prophesee Gen3.1} & {640 × 480} & {59.9} & {60.1}\\
\hline
\end{tabular}
}
\label{tab:1}
\vspace{-1.5em}
\end{center}
\end{table}
